Guillotine: Hypervisors for Isolating Malicious AIs

As AI models become more embedded in critical sectors like finance, healthcare, and the military, their inscrutable behavior poses ever-greater risks to society. To mitigate this risk, we propose Guillotine, a hypervisor architecture for sandboxing powerful AI models -- models that, by accident or malice, can generate existential threats to humanity. Although Guillotine borrows some well-known virtualization techniques, Guillotine must also introduce fundamentally new isolation mechanisms to handle the unique threat model posed by existential-risk AIs. For example, a rogue AI may try to introspect upon hypervisor software or the underlying hardware substrate to enable later subversion of that control plane; thus, a Guillotine hypervisor requires careful co-design of the hypervisor software and the CPUs, RAM, NIC, and storage devices that support the hypervisor software, to thwart side channel leakage and more generally eliminate mechanisms for AI to exploit reflection-based vulnerabilities. Beyond such isolation at the software, network, and microarchitectural layers, a Guillotine hypervisor must also provide physical fail-safes more commonly associated with nuclear power plants, avionic platforms, and other types of mission critical systems. Physical fail-safes, e.g., involving electromechanical disconnection of network cables, or the flooding of a datacenter which holds a rogue AI, provide defense in depth if software, network, and microarchitectural isolation is compromised and a rogue AI must be temporarily shut down or permanently destroyed.

==> abstract.tex <==
As AI models
become more embedded in
critical sectors like
finance, healthcare, and the military,
their inscrutable behavior
poses ever-greater risks to society.
To mitigate this risk,
we propose \system,
a hypervisor architecture
for sandboxing powerful AI models---models that,
by accident or malice,
can generate existential threats to humanity.

==> conclusion.tex <==
\label{sec:conclusions}

!!!Write me

!!!Maybe talk about how \system can be used during model \textit{training} as well. As Greenblatt et al. described~\cite{greenblatt2024}, a model can fake compliance with alignment goals during training. This raises the possibility that, during training, a model can attempt more active kinds of maliciousness.

==> hypervisor-policy.tex <==

\subsection{Policy Hypervisor}
\label{sec:hypervisor-policy}
 
\epigraph{
1 – A robot may not injure a human being, or, through inaction, allow a human being to come to harm. \\ 
2 – A robot must obey the orders given it by human beings except where such orders would conflict with the First Law. \\ 
\st{3 – A robot must protect its own existence as long as such protection does not conflict with the First or Second Law.} \\ 
Handbook of Robotics, 56th Edition, 2058 A.D.}
{\textit{iRobot, Asimov\\Third law deleted by the authors of this paper.}}


Preexisting law and policy define what makes an AI model ''risky".
\system is best-suited for general-purpose models which pose ''systemic risk", as defined by the EU AI Act. 
Examples of such systemic risks include the ability to contribute to nuclear weapon attacks, cyberattacks on critical infrastructure, or degradation of human rights (3.2, EU CoP Draft 2~\cite{CITE}).
Under EU legislation, a model's systemic risk is estimated using criterion from model development, such as parameter counts and training benchmarks used (Annex 13, EU AI Act), as well as features of the model, such as its cyber-offensive capabilities or level of autonomy (3.4.1, EU CoP Draft 2 ~\cite{CITE}).

The EU AI Act requires the providers of models posing systemic risk to comply with reporting guidelines; for example, providers must give the European Commission technical documentation and model source code when requested (Article 92, EU AI Act~\cite{CITE}). 
We propose operators should similarly be required to use (and report on their use of) \system hypervisors. 
Government organizations could specifically implement auditing mechanisms, which allow companies to prove what level of \system they are running for a given model, similar to enforcement mechanisms for web certificates~\cite{mozilla, google} and nuclear weapon adherence mechanisms~\cite{start}. 
As with current AI legislation, governments could implement fines for non-compliance.

We believe the increased cost and effort associated with \system may be justified by model deployers by including \system in a ''Safe Harbor" framework.
In this ''Safe Harbor", companies face reduced legal liability if a model leads to a certain subset of systemic harms (i.e., a cyberattack), as long as they had correctly implemented \system, and complied with government audits. 
This implementation aligns incentives of regulators and model deployers, as organizations receive legal protection in exchange for the added cost associated with \system. 


==> related-work-systems.tex <==
%jwm: I'm not including this part in the draft
%     for space reasons, and because we cover
%     the basics of some of this material earlier
%     in the paper.

\noindent
\textbf{Microarchitectural isolation:}
The goal of the \system microarchitectural-level hypervisor
is to strongly isolate the software-level hypervisor
from an untrusted AI model.
\system does so
by eliminating microarchitectural co-tenancy,
willingly paying a cost in die area
in exchange for eliminating side channels by definition.
Traditional in-silicon mechanisms
for enclave execution~\cite{!!!sgx,!!!amd-sv,!!!risc-v}
and hypervisor-based isolation~\cite{!!!}
provide strong ISA-level isolation
between software from different trust domains;
however,
these approaches
typically use the same underlying microarchitecture
to run both types of code,
making these systems vulnerable
to side channel attacks~\cite{!!!surveyOfSideChannelAttacks}.

In contrast,
MI6 enclave-aware processors~\cite{mi6}
partition DRAM and the L1--L3 caches,
giving each enclave
a dedicated slice of the memory hierarchy
to avoid side channels via that hierarchy.
MI6 also uses a DRAM controller
that provides constant-time latency,
eschewing optimizations like request reordering
that increase DRAM bandwidth
but enable side channels.
When a core transitions from
enclave mode to non-enclave mode,
MI6 explictly purges microarchitectural state
like branch predictors and L1 caches;
pinning enclaves to cores
can reduce the number of MI6 transitions~\cite{ironhide}.
\system's approach of
using dedicated model cores
with dedicated memory hierarchies and
no context switches
enables better performance
but requires more die area.

An undervisor-aware processor~\cite{undervisor}
runs a monitor program for an enclave
on a pipeline
that is microarchitecturally inaccessible
to the enclave.
The monitor pipeline
runs in parallel to the enclave pipeline
and can examine the register state,
instruction stream,
and instruction operands and results
from that pipeline.
However,
the monitor cannot examine
arbitrary memory state belonging to the enclave,
and has restricted expressivity.

\noindent
\textbf{Physical isolation:}
Datacenter security companies
like Valiant, Airgap, and Goldilock
have proposed ``network kill switches''
as a way to limit attacker mobility
once a datacenter breach has occurred~\cite{valiantKillSwitch,airgapKillSwitch,
goldlockKillSwitch}.
The basic idea
is to divide a datacenter network
(and its associated servers)
into zones;
when the datacenter operator
detects the compromise
of servers in a particular zone,
the operator can
cut that zone off
from the rest of the datacenter network,
preventing the attacker
from subverting additional machines.
Airgap and Valiant kill switches
are implemented as
Layer 2 network appliances,
with network disconnection enforced
via on-device routing software.
In contrast,
Goldilock kill switches
are logically equivalent to
Layer 1 pass-through cables,
with network severing implemented via
physical disconnection of
electromechanical Reed switches~\cite{goldlockFAQ,reedSwitch}.
Airgap, Valiant, and Goldilock devices
receive kill commands via
dedicated serial ports or Ethernet ports,
via SSH connections
that traverse standard Ethernet ports,
or (in the case of Goldilock)
via SMS messages
sent from trusted phone numbers.
